Charting the Future: Using Chart Question-Answering for Scalable Evaluation of LLM-Driven Data Visualizations

We propose a novel framework that leverages Visual Question Answering (VQA) models to automate the evaluation of LLM-generated data visualizations. Traditional evaluation methods often rely on human judgment, which is costly and unscalable, or focus solely on data accuracy, neglecting the effectiveness of visual communication. By employing VQA models, we assess data representation quality and the general communicative clarity of charts. Experiments were conducted using two leading VQA benchmark datasets, ChartQA and PlotQA, with visualizations generated by OpenAI's GPT-3.5 Turbo and Meta's Llama 3.1 70B-Instruct models. Our results indicate that LLM-generated charts do not match the accuracy of the original non-LLM-generated charts based on VQA performance measures. Moreover, while our results demonstrate that few-shot prompting significantly boosts the accuracy of chart generation, considerable progress remains to be made before LLMs can fully match the precision of human-generated graphs. This underscores the importance of our work, which expedites the research process by enabling rapid iteration without the need for human annotation, thus accelerating advancements in this field.

==> bakup.tex <==


\begin{comment}
Data analytics play an essential role in modern organizations, and effective data visualization is crucial for translating complex information into actionable insights. As the availability of business intelligence has expanded with the rise of big data, organizational staff are often overwhelmed by the sheer volume and complexity of information. However, many individuals lack the technical expertise to generate visualizations supporting informed decision-making.



Despite this progress, evaluating the quality of LLM-generated visualizations presents a challenge. Current evaluation methods typically rely on human judgment, requiring evaluators to assess both the data accuracy and the overall communication effectiveness of the visualizations. This reliance on human assessment is not only costly but also difficult to scale across large datasets or diverse visualizations. Moreover, human evaluations are subjective, prone to variability, and time-consuming, making it impractical for continuous system development or large-scale benchmarking.

An alternative approach is to regenerate the input data from the visualization and compare it to the original dataset. However, this method has fundamental limitations. First, it focuses solely on the accuracy of the data representation, ignoring other critical factors, such as the clarity of visual design, the ease of interpretation, and whether the visualization effectively highlights key insights. Moreover, it does not measure if simple aspects are correct, e.g., if a bar chart is supposed to be created, but a line plot is used instead; measuring data recreation accuracy does not help. For example, a chart might accurately represent the underlying data but fail to convey the intended trend due to poor color choices, confusing labels, or cluttered layouts. In such cases, regenerating the data would not reveal these issues, as it only checks whether the data matches, rather than evaluating how well the visualization communicates the information.


\begin{figure}[t]
    \centering
    \includegraphics[width=.8\linewidth]{fig-plot.pdf}
    \caption{VQA Process}
    \label{fig:enter-label}
\end{figure}

In contrast, visual question answering (VQA) offers a more nuanced approach to evaluating visualizations. VQA models are capable of answering questions about both the data and the design elements of a chart, providing a richer understanding of its effectiveness~\cite{liu-etal-2023-matcha, masry-etal-2023-unichart}. For example, a VQA model could answer questions like, "What trend is depicted in this chart?" or "Which category shows the highest value?"—questions that evaluate the user's interpretation of the visualization rather than just verifying the underlying data. This feedback is particularly useful because it addresses the ultimate goal of a visualization: to communicate insights effectively, which regenerating the data alone cannot capture.


Moreover, VQA allows for scalable, automated evaluation, reducing the dependency on human evaluators and enabling large-scale assessments across various visualization types. By focusing on visualizations' interpretability and design aspects, VQA provides an evaluation method closer to how end-users interact with and interpret visual content in real-world scenarios. An example of the VQA process is provided in Figure 1.

In this paper, we introduce a novel framework that leverages chart-based VQA models to automate the evaluation of LLM-generated visualizations at scale. Specifically, we make the following contributions: 1) We demonstrate how VQA models provide unique, context-sensitive feedback compared to data regeneration methods, offering a more holistic assessment of both data accuracy and visual communication; 2) We develop an automated framework that scales the evaluation of LLM-generated visualizations without requiring human intervention; and 3) We present empirical results showcasing the effectiveness of our approach in large-scale evaluations benchmarking multiple large language models using different prompting strategies. The following sections will review relevant literature, outline our experimental design, present preliminary findings, and discuss future directions.

Natural language data analysis systems have existed for numerous years, evolving from rule-based or template-based methods and shallow parsing techniques~\cite{9699035,10530359}. Such systems struggled with complex data and had limited efficacy~\cite{hong2023conversationalaithreadsvisualizing}.  The rise of natural language processing and deep learning models led to improvements in complexity and robustness, but such systems required extensive training data pertinent for the desired tasks~\cite{10530359, 10443572}.  Only recently have LLM models begun to be applied to generation of data visualizations. 
However, the issue of evaluating these methods has not been adequately addressed. Much of the research requires human evaluation, so the results can not be scaled without significant costs. 
Traditionally, three types of evaluation metrics were employed: comparing the generated code to ground-truth specifications, comparing generated visualizations with expected outputs, and/or perceptual ratings of user satisfaction~\cite{10530359}.  In addition, case-study methods have been employed with the analysis conducted by the authors~\cite{10121440}.
Conceptual frameworks for evaluation of LLM-generated visualizations have been proposed which automates some portions of the evaluative process, but the human element still remains~\cite{10344146, podo2024vievallmconceptualstack}.
Thus, the primary limitation of previous evaluation efforts remains the necessity of human participation, increasing the costs and reducing the scope.

Yet, much progress has been made with research regarding visual question-answering (VQA), specifically in terms of chart visualizations~\cite{liu-etal-2023-matcha, masry-etal-2023-unichart}. These models take an existing digital plot and answer questions about the information conveyed as well as the layout and characteristics of the plot. VQA offers a possible method of evaluating LLM-generated visualizations at scale. The contribution of this research will be to develop an automated method to conduct evaluations of LLM-generated visualizations at scale through the use of chart question-answering models. The following sections will present an overview of the relevant research on these topics, detail the experimental design and preliminary results, and outline proposed future steps.

Summarizing, the contributions of this paper are: (1) a method of applying VQA techniques to automate the evaluation of LLM-generated data visualizations; (2) a comprehensive experiment comparing automated evaluation compared to human evaluation across multiple models and data sets.
\end{comment}


\begin{comment}
While data visualization allows for greater and faster understanding of insights from the figures and text, creating such plots can be complex and require numerous steps. These include becoming familiar with the dataset and its structure, understanding the goals or insights desired from the data, choosing the most appropriate visualization type and layout, and then either writing code or utilizing another user interface to produce the output~\cite{10.2312/eurovisshort.20171133,dibia-2023-lida}.

Natural language interfaces (NLI)--also referred to as Text-to-Viz--for data visualization efforts involve taking users’ natural language input as well as a data source in order to generate desired charts and plots. Prior to the development of Text-to-Viz, interactive visualization required the use of Windows, Icons, Menus, and Pointer (WIMP) interface tools, necessitating technical expertise to be used effectively~\cite{9699035}. Complex data and intricate visualization output require systems with steep learning curves, and non-technical users face challenges in choosing the correct procedures to best analyze and present their results~\cite{app13127025}. Various commercial data analysis and reporting tools such as Tableau, Microsoft Power BI, and IBM Watson Analytics have implemented limited NLI capabilities to varying degrees in their products~\cite{10121440}.

NLIs consist of two components, tabular data querying and visualization, so that users can retrieve data from sources such as SQL-based databases and display the results in charts and graphs~\cite{affolter_comparative_2019,10530359}. Note that for the purposes of this research, the focus will only be on the second component. Even so, the task requires multiple steps, including parsing the input query, identifying data attributes, conducting any necessary analyses, choosing the appropriate visualization style, and then generating code \cite{10121440}.

The use of NLI is intended to increase such factors as user convenience and novice-friendliness, intuitiveness and effectiveness, and humanistic care (inclusiveness for non-visual access) ~\cite{9699035}. Challenges of such applications include ambiguity and under-specification in natural language, conversational context complexity, and limited discoverability of system capabilities (Ibid). In addition, users tend to overestimate the capacity of the NLI tool in understanding the natural language utterance, with expectations that are unrealistic and thus not met~\cite{8986918}. Users expect systems to interpret their requests in context, which is difficult when the initial query is under-specified.

\subsection{Classic NL2Viz}

Natural language data analysis systems have been developed for more than two decades~\cite{9699035}.  As early as 2001, a prototype was developed which required structured queries ~\cite{cox_multi-modal_2001}. Early NLI for data visualization relied on rule-based or template-based systems and shallow parsing methods, struggling with complex data~\cite{10530359}. While these methodologies are still in use in commercial NLI systems, they have had limited efficacy ~\cite{hong2023conversationalaithreadsvisualizing}. 

Approximately ten years ago, development of techniques such as word embeddings and neural network methods spurred new NLI data visualization systems ~\cite{9699035}. Sequence-to-sequence models allowed for more complexity and robustness, but required extensive training data, while pre-trained language models such as BERT and T5 provided more capabilities in applying NLP to visualizations~\cite{10530359, 10443572}. For example,~\citet{voigt-etal-2023-vist5} and~\citet{10443572} utilized FLAN-T5-based models to create Vega-Lite specifications for data visualizations. ~\citet{10.1145/3534678.3539330} split the process into separate visualization retrieval network and query revision network models. 

The development of the toolkit NL4DV allowed for the creation of Vega-Lite chart specifications from natural language queries directly from Python applications~\cite{9222342}. More recently, interactive systems have been developed which combine text and speech inputs along with traditional mouse and keyboard interfaces~\cite{10.1145/3313831.3376782, 9303381} 

\subsection{LLM2Viz}

The recent rise in LLM models has witnessed various attempts to harness their power to create data visualizations from natural language inputs. LLMs have performed well in tasks ranging from generation of text, code, and images as well as image captioning, so visualization applications are within their capabilities~\cite{dibia-2023-lida}. LLMs promise increases in accuracy in terms of comprehending user queries, even when under-specified~\cite{10121440}. In comparison to deep learning methods, LLM techniques do not require extensive pre-training efforts \cite{hong2023conversationalaithreadsvisualizing}.  Research has shown that LLM models match the performance of human data analysts~\cite{cheng-etal-2023-gpt}, although various challenges and obstacles remain~\cite{zhang2024benchmarkingdatascienceagents,gu2024analystsunderstandverifyaiassisted}.

Some of these LLM applications generate actual chart images while others create Python, Vega-Lite, Javascript, or other coding language which can produce specific plots when executed ~\cite{podo2024vievallmconceptualstack}. Rather than fine-tuning NLP models, these efforts typically focus on prompt-engineering to output the visualizations. More recent efforts have introduced methods such as chain-of-thought processes to increase the efficacy of the visualizations.

~\citet{chen2022nl2interfaceinteractivevisualizationinterface} used OpenAI Codex to generate Structurally Parameterized SQL to create visualization interfaces.  ~\citet{10121440} employed OpenAI models (Davinci, Codex, and ChatGPT) to generate Python scripts. ~\citet{li2024visualizationgenerationlargelanguage} implemented few-shot prompt strategies to compare different prompt-engineering results, using GPT-3.5 and Vega-Lite.~\citet{dibia-2023-lida} as well as ~\citet{hong2023conversationalaithreadsvisualizing} and~\citet{10458347} developed user interfaces to upload datasets, examine the data, create visualizations, and refine the output. ~\citet{podo2024vrecslowcostllm4visrecommender} developed a chain-of-thought process combined with a large LLM (GPT-4) serving as a teacher instructing a smaller LLM (Llama-2-7B) as a student, in order to minimize computational costs.

\subsection{Evaluation of LLM2Viz}

Evaluation of NLI visualizations traditionally is based on three types of metrics~\cite{10530359}. String-based measurement compares the generated code or specifications to ground-truth specifications, and can be exact match or component match. Execution-based measurement similarly compares the generated result with the desired output. Manual measurement rates the user satisfaction with the interface and usability.

The LLM2Viz research has indicated that LLM-generated visualizations are prone to hallucinations ~\cite{podo2024vievallmconceptualstack, 10443572}. In addition, LLM output has evidenced inconsistency when the same prompts were executed on the same data~\cite{10121440}. ~\citet{ijgi12070284} found that LLM-generated map data visualizations depended heavily on user interventions for quality control purposes.

Some of the studies evaluated the model output through a case study approach, with the authors analyzing the results. For example,~\citet{10121440} devised six case studies to determine how accurate and effective the visualizations were. Much of the evaluation of the results were done through small-scale user studies rather than automated processes.~\citet{10458347} surveyed a small group of users, and \citet{hong2023conversationalaithreadsvisualizing} conducted both a usability survey with users as well as interviews with a panel of experts to gather qualitative feedback. Extensive research has addressed factors regarding qualitative feedback and user studies~\cite{9118800}. 

In terms of evaluation of LLM-generated visualizations, recent research has employed mixed-method techniques to combine quantitative and qualitative results.~\citet{10344146} tasked GPT-3.5 and GPT-4 with assignments from an undergraduate data visualization course to assign a student grade in completing the class requirements, as well as qualitative feedback from a panel of experts, judging on abilities regarding data interpretation, visualization design, visual exploration, and communication of insights. ~\citet{li2024visualizationgenerationlargelanguage} compared zero-shot with few-shot prompting methods, evaluating them based on a text analysis of the GPT-3.5-generated Vega-Lite specifications, judging whether the chart type and data included in the visualizations matched the ground truth from the existing dataset.~\citet{dibia-2023-lida} combined accuracy metrics with a self-rating generated by GPT-4 to assess the visualization quality across six dimensions: code accuracy, data transformation, goal compliance, visualization type, data encoding, and aesthetics.

~\citet{podo2024vievallmconceptualstack} introduced a conceptual framework for the evaluation of LLM-generated visualizations, combining manual and automated scoring. The framework addresses such factors as code correctness and coherence (Code layer), data mapping and axes/mark correctness (Representation layer), color mapping and perceptual quality (Presentation layer), visualization literacy and significance (Informativeness layer), and LLM effort (LLM layer). While these layers are evaluated with a combination of human and automated methods depending on the factor, the authors propose a LLM to be an additional evaluator.  Building on this effort, ~\citet{10670425} applied an evaluation framework in order to compare a series of LLM models.  The visualizations were measure for dimensions including validity, legality, and readability.

Thus, current evaluation approaches tend to rely on user studies and/or expert panels in order to qualitatively rate the visualization outputs. Automated efforts primarily focus on checking the syntax of the generated code~\cite{8744242}, and, more recently, having LLM models provide self-ratings.  Note, however, that some research has indicated that code similarity may not be a good indicator~\cite{10670425}, and that human feedback was preferred to LLM feedback~\cite{kim2024goodchatgptgivingadvice}.

\subsection{Visual Question-Answering}

However, VQA research streams offer a possible solution to resource-heavy manual evaluation or computing-cost expensive LLM self-rating. The models accurately answer one or more questions concerning a data chart, allowing a method of evaluating generated visualizations at scale. The questions typically involve factoids from the chart using visual and arithmetic reasoning~\cite{masry-etal-2023-unichart}.  Two methods of analyzing the charts include either converting the data into underlying tables and then using text analysis of the resulting tables, or using multimodal models to derive the answers from the chart itself~\cite{han2023chartllamamultimodalllmchart}.

Two of the primary benchmark datasets for VQA in recent years has been ChartQA~\cite{masry-etal-2022-chartqa} and PlotQA~\cite{Methani_2020_WACV}. ChartQA is comprised of more than 32,000 question-answer pairs based on approximately 21,000 real-world charts obtained from sources such as Statista, Pew Research, Our World in Data, and the Organization for Economic Co-operation and Development (OECD), regarding topics ranging from economics to demographics to social and political issues. For the questions-answer pairs, nearly 10,000 were human-written and the remaining two-thirds were augmented through the use of a T5 model to automatically generate from chart summaries. The human-authored questions are typically more complex and difficult to answer, using more visual and logical reasoning with varied language than the augmented questions.

PlotQA consists of nearly 30 million question-answer pairs from approximately 225,000 charts. The charts are real-world, coming from sources such as the World Bank and governmental agency websites. Questions are categorized into Data Retrieval, Structural, and Reasoning (Arithmetic, Comparison, Compound, or Min-Max) types. Structural questions refer to the overall structure (e.g. number of bars or lines in the chart) without requiring any quantitative reasoning, while Data Retrieval questions ask for the data of a single element such as the count or percentage that a bar represents. Reasoning questions involve numeric reasoning and/or comparisons across multiple elements in the chart, an example of which would be how much higher is one bar’s percentage than another or which are the highest or lowest bars.

Both datasets have been extensively utilized in subsequent research to improve VQA performance. ~\citet{masry-etal-2023-unichart} developed Unichart, a model with two modules (a chart encoder based on the document image Donut model, plus a text decoder based on a BART model) pre-trained on more than 600,000 charts. Unichart inputs a plot image and encodes the text elements (legends and axis labels), visual elements (bars and lines), and the layout of the plot and next decodes the text for answer generation.~\citet{liu-etal-2023-matcha} created MatCha, adding chart derendering and mathematical reasoning pretraining to the Pix2Struct vision-language model. Both Unichart and Matcha reported high performance on VQA with the ChartQA and PlotQA datasets.
\end{comment}






\begin{comment}This research utilized LLMs to create data visualizations. Two LLM models were used to generate the charts, OpenAI GPT-3.5 Turbo-0125 and neuralmagic Meta Llama 3.1 70B-Instruct-FP8. 

Data files in text format were loaded and passed to the LLMs along with prompts to generate Python Matplotlib code to create the charts. The data files consisted of samples from the ChartQA and PlotQA benchmark datasets. To evaluate, question-answer pairs from the two benchmark datasets were applied to the generated charts and the existing dataset charts, using the respective Unichart and MatCha VQA models, to compare the accuracy. A zero-shot prompt formed the baseline and then few-shot prompting versions were compared.

The sample from each dataset consisted of underlying CSV data files, charts, and question-answer pairs. A total of 1,134 samples from the validation sets were selected for the analysis, resulting in 15,540 question-answer pairs. Table 1 details the sample breakout from the two datasets.


The initial zero-shot prompt contained these instructions:

{"role": "system", "content": "You are a data analyst tasked with creating the data visualization plots to best match the data provided. Output should be formatted as python matplotlib code and add both fig.clf() and the bbox-inches=tight parameter. Title, chart type and the data are given in the user instructions. Be sure to set up the X and Y data elements as provided in terms of axis label names as well as counts, so do not use list(range). Put data value labels on the chart, place any legends outside of the chart pane, and the chart should be output to a png file using the filename in the user instructions."}

{"role": "user", "content": data-pass}

where 

data-pass = "Title: " + title-text + " / Data: " + final-string +" / Chart type: " +
figure-type + " / File Name: " + png-file

The few-shot prompt added two examples of similar chart information along with generated Python code to produce charts.

The evaluation tested whether a difference in accuracy exists when the VQA models are applied to the existing dataset charts from each sample versus the LLM-generated charts. Accuracy is defined as the answer from the VQA models matching the ground truth in the dataset. For text responses, strict accuracy was employed but relaxed accuracy~\cite{masry-etal-2022-chartqa} was used for mathematical and numerical responses. Relaxed accuracy is operationalized as accepting numerical values that are within plus or minus five percent.  In addition, data extraction analysis was performed using the DePlot model~\cite{liu-etal-2023-matcha} to evaluate whether the generated charts utilized the same data data as the ground truth files.
\end{comment}



\begin{table*}
  \centering
  \begin{tabular}{l r r}
    \hline
    \textbf{Dataset / Model} & \textbf{Similarity Score} & \textbf{Exact Match} \\
    \hline
    \verb|ChartQA Existing|     & 97.8\    & 70.6\     \\
    \verb|ChartQA ChatGPT Zero-Shot|  & 97.0\    & 30.8\              \\
    \verb|ChartQA Llama 3.1 Zero-Shot|     & 95.3\    & 33.1\     \\
    \verb|ChartQA ChatGPT Few-Shot|     & 97.2\    & 43.5\     \\
    \verb|ChartQA Llama 3.1 Few-Shot|     & 97.7\    & 43.5\     \\
    \verb|PlotQA Existing|     & 92.2\    & 16.0\     \\
    \verb|PlotQA ChatGPT Zero-Shot|  & 92.5\    & 49.3\              \\
    \verb|PlotQA Llama 3.1 Zero-Shot|     & 82.7\    & 25.0\     \\
    \verb|PlotQA ChatGPT Few-Shot|     & 92.3\    & 37.0\     \\
    \verb|PlotQA Llama 3.1 Few-Shot|     & 93.1\    & 35.8\     \\
    \hline
  \end{tabular}
  \caption{Data Extraction Results Using DePlot}
  \label{tab:accents}
\end{table*}



\begin{comment}The findings indicate that while the LLM-generated charts do not provide quite the accuracy of the original existing charts from the dataset, a few-shot approach does improve the resulting accuracy. Tables 2 and 3 compares the existing charts versus the LLM-generated charts in terms of VQA accuracy. The Unichart VQA model ~\cite{masry-etal-2023-unichart} was applied to the the ChartQA dataset while the MatCha VQA model~\cite{liu-etal-2023-matcha} was applied to the PlotQA data, the datasets for which each were fine-tuned. With the zero-shot baseline, the LLM-generated results did not match the accuracy of benchmark datasets.  However, the few-shot provides a strong improvement especially with the Llama 3.1 model. The ChatGPT 3.5 Turbo charts performed worse than the Llama 3.1 70B charts on the ChartQA dataset but better on the PlotQA set.



Interestingly, the results differed by type of question. As stated in the Literature Review section, the Human questions in the first dataset are more complex than the Augmented questions, with more complicated reasoning required and more variation in wording. For the PlotQA dataset, some question types were more accurately answered than others. Arithmetic calculations had the lowest rating, while Min-Max, Structural and Comparison categories were highly accurate. For the ChartQA dataset, the Llama 3.1 results were actually more accurate than the original versions for the human created questions once the few-shot method was applied.

In terms of the data extraction task, two methods were used to evaluate the results.  The first method, adapted from ~\citet{masry-etal-2023-unichart} and labeled "Similarity Score" on Table 4, uses the normalized distance between the extracted values from each LLM-generated chart and the ground truth data files.  The second method, labeled "Exact Match", computes the percentage of charts whose extracted data tables are exact matches with the ground truth tables.  The DePlot data extraction model~\citet{liu-etal-2023-matcha} was used for both datasets.  The results were reversed from the VQA findings, with the ChatGPT 3.5 Turbo charts performing better than the Llama 3.1 70B charts.

Reviewing the actual charts generated by the LLM, a number of them did display hallucinatory results or were otherwise incorrect. There were instances where elements of the x or y-axis labels were truncated, omitted, or referred to text not appearing in the prompt passed to the LLM.

Human evaluation results indicated that the ChatGPT and Llama LLMs performed similarly, with the former scoring slightly higher in some aspects and slightly lower in others. Table 5 displays the results, as scored on the 5-point Likert scale detailed above.  Both models scored higher on accuracy metrics than on the ease of understanding, visual appeal, and satisfactory metrics.
\end{comment}

